Separators in region intersection graphs

For undirected graphs $G=(V,E)$ and $G_0=(V_0,E_0)$, say that $G$ is a region intersection graph over $G_0$ if there is a family of connected subsets $\{ R_u \subseteq V_0 : u \in V \}$ of $G_0$ such that $\{u,v\} \in E \iff R_u \cap R_v \neq \emptyset$. We show if $G_0$ excludes the complete graph $K_h$ as a minor for some $h \geq 1$, then every region intersection graph $G$ over $G_0$ with $m$ edges has a balanced separator with at most $c_h \sqrt{m}$ nodes, where $c_h$ is a constant depending only on $h$. If $G$ additionally has uniformly bounded vertex degrees, then such a separator is found by spectral partitioning. A string graph is the intersection graph of continuous arcs in the plane. The preceding result implies that every string graph with $m$ edges has a balanced separator of size $O(\sqrt{m})$. This bound is optimal, as it generalizes the planar separator theorem. It confirms a conjecture of Fox and Pach (2010), and improves over the $O(\sqrt{m} \log m)$ bound of Matousek (2013).

==> macros-notes.tex <==

% abbreviations and paper-specific macros

\let\pref=\prettyref

\renewcommand{\Vsymb}{\mathrm{Var}}

% \setlength{\parskip}{2pt}

\newcommand{\PP}{\mathfrak{P}}
\newcommand{\sos}{\mathsf{sos}}
\newcommand{\cone}{\mathrm{cone}}
\newcommand{\gap}{\mathrm{gap}}
\let\super\varsuper
\newcommand{\ML}[2]{\mathrm{\cQ}^{#2}_{#1}}
\newcommand*{\id}{\mathrm{id}}
\newcommand{\Cay}{\mathsf{Cay}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\dmid}{\,\|\,}
\newcommand{\D}{\mathbb{D}}
\DeclareMathOperator{\tr}{tr}
\newcommand{\Lone}[1]{\left\|#1\right\|_1}
\newcommand{\Linf}[1]{\left\|#1\right\|_{\infty}}

\newcommand*{\qe}[2]{S(#1\,\|\, #2)}
\newcommand*{\ce}[2]{D(#1\,\|\, #2)}

\newcommand*{\sst}{\substack}

\ifnum\arxivmode=0
\renewcommand{\Ind}{\vvmathbb{1}}
\else
\renewcommand{\Ind}{\bm{1}}
\fi
\ifnum\jamesmode=0
% \renewcommand{\Ind}{\vvmathbb 1}
\fi
\let\1\Ind

\newcommand*{\hi}{\mathsf{high}}
\newcommand*{\low}{\mathsf{low}}

\newcommand*{\inst}{\Im}
\newcommand*{\GF}[1]{\mathbb F_{#1}}

\newcommand\f{\varphi}
\newcommand{\F}{\mathcal F}
\newcommand{\OR}{\ensuremath{\mathsf{OR}}}
\newcommand*{\gtwo}{\gamma_{2\to 2}^{\mathsf{psd}}}
\newcommand*{\psdrank}{\mathrm{rank}_{\mathsf{psd}}}
\newcommand*{\psdalpha}{\alpha_{\mathsf{psd}}}
\newcommand*{\nnalpha}{\alpha_{+}}
\newcommand{\psd}{\mathsf{psd}}
\newcommand*{\apsdrank}{\rho_{\mathsf{psd}}}
\newcommand*{\nnrank}{\mathrm{rank}_{+}}
\newcommand*{\sosdeg}{\deg_{\mathsf{sos}}}
\newcommand*{\juntadeg}{\deg_{+}}

\newcommand{\polytope}[1]{\text{\textup{\textsc{#1}}}}

\newcommand*{\corr}{\polytope{corr}}
\newcommand*{\tsp}{\polytope{tsp}}
\newcommand*{\cut}{\mathsf{cut}}
\newcommand*{\stab}{\polytope{stab}}

\newcommand*{\ot}{\otimes}
\newcommand*{\pmo}{\{\pm 1\}}


\newcommand*{\maxpi}{\problemmacro{max-$\Pi$}}
\newcommand*{\maxscrP}{\problemmacro{max-$\scrP$}}
\newcommand*{\maxthreecnf}{\problemmacro{max \pnum{3}-cnf}}


% \newcommand*{\pE}{\tilde {\mathbb E}}

\newcommand*{\sleq}{\preceq}
\newcommand*{\sgeq}{\succeq}

\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\argmin}{\mathrm{argmin}}
%\DeclareMathOperator{\argmax}{\mathrm{argmax}}

\DeclareMathOperator{\pE}{\tilde {\mathbb E}}

% uniform density operator

% \newcommand*{\uId}{\tfrac 1 {\Tr \Id}\Id}
\newcommand*{\uId}{\mathcal{U}}

\newcommand*{\annotaterel}[2]{\stackrel{\scriptscriptstyle\text{#1}}{#2}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sdpsize"
%%% End:

